Weight-based Decomposition: A Case for Bilinear MLPs

Gated Linear Units (GLUs) have become a common building block in modern foundation models. Bilinear layers drop the non-linearity in the "gate" but still have comparable performance to other GLUs. An attractive quality of bilinear layers is that they can be fully expressed in terms of a third-order tensor and linear operations. Leveraging this, we develop a method to decompose the bilinear tensor into a set of sparsely interacting eigenvectors that show promising interpretability properties in preliminary experiments for shallow image classifiers (MNIST) and small language models (Tiny Stories). Since the decomposition is fully equivalent to the model's original computations, bilinear layers may be an interpretability-friendly architecture that helps connect features to the model weights. Application of our method may not be limited to pretrained bilinear models since we find that language models such as TinyLlama-1.1B can be finetuned into bilinear variants.

==> files/abstract.tex <==



==> files/intro_alice.tex <==
% Alice scratch pad

% Lead with mech interp as the focus, rather than MNIST
% Mechanistic interpretability is posed
% Also introduce bilinear layers
Multi-Layer Perceptrons (MLP) are ubiquitous components of large language models (LLMs) and deep learning models generally. Because of their nonlinear activation function, MLPs have historically been treated as irreducible components in mechanistic interpretability \cite{elhage_mathematical_2021, black_interpreting_2022}. 
% cite mathematical framework, polytope lens, mnist failure
% For example, until now there has been no mechanistic account of how MLPs classify MNIST digits.
Nonlinear activations are a major limitation because 1) they introduce complicated interactions (typically of all orders) between input features and 2) the neurons act as a priliveged basis \cite{elhage_toy_2022, brown2023privileged}, so we cannot transform to a feature basis and cannot easily work with linear combinations of neurons. MLPs have only been well-understood in special cases such as small networks trained on math problems \cite{nanda2022progress, chughtai2023toy, michaud2024opening}. 

Recent interpretability work does not rely on parsing model weights. Instead, sparse autoencoders (SAEs) are used to derive interpretable features based on a model's internal activations over a dataset \cite{cunningham_sparse_2024, bricken_monosemanticity_2023, marks2024sparse}. Training transcoders to bridge features from one layer to those in the next ends up circumventing MLPs entirely \cite{dunefsky2024transcoders, sparsify}. Although SAE-based approaches have been successful, there remain questions about their data dependency and their behavior out-of-distribution. Ideally there would be a way to connect the SAE-derived features to the model's computations.
 
Another approach is to use a more interpretable architecture. \citet{bilinear_note} suggested that bilinear MLP layers of the form $g(x) = (W\mathbf{x}) \odot (V\mathbf{x})$ have advantages for interpretability because their computations can be expressed in terms of linear operations with a third order tensor. This allows us to leverage tensor or matrix decompositions to understand the weights. A comparison of activations found that bilinear activations outperformed ReLU and GELU in transformer models \cite{shazeer2020glu}, and have performance only slightly below SwiGLU, which is prevalent in competitive open source transformers today.

This paper aims to provide a demonstration of how bilinear MLP layers can be decomposed into a set of functionally relevant features. We use the word ``feature'' loosely to describe linear directions in activation space that appear interpretable, even if they are not necessarily sparse. Our contributions are as follows:

\begin{enumerate}
    \item We introduce a method to decompose bilinear MLPs into a set of eigenvector features with sparse interactions. This decomposition is fully equivalent to the layer's original computations. It is possible to chain these decompositions together to decompile a deep MLP-only model.
    \item In shallow image classification (MNIST) models, we show that the top eigenvectors are interpretable, and smaller eigenvalue terms can be truncated while preserving performance. Weight decay and noisy training produce qualititatively more interpretable features.
    \item Preliminary results on small language models (Tiny Stories) suggest that language eigenvectors can also interpretable. We give evidence that larger pretrained language models can be finetuned into bilinear models using little data, to achieve loss similar to that expected from pretraining.
    %\item For shallow image classification (MNIST) models we demonstrate that the top eigenvectors are largely interpretable. Preliminary results for a small language model (Tiny Stories) also suggests their interpretability. 
    %\item We show that foundation models can be finetuned into bilinear models using little data, achieving loss similar to that expected from pretraining. 
\end{enumerate}
We open-source our code and provide notebooks to replicate all experiments (we will provide a link here if accepted).
%Multi-Layer Perceptrons (MLP) pose a major limitation to mechanistic interpretability, and are often omitted in circuit analyses found in literature because of this. Non-linearities are crucial for model performance, but they introduce data dependent activations. Although sparse auto-encoders (SAE) have had success, they depend on an additional training run (costly) and their features might depend on the dataset used. It is possible that out-of-distribution (OOD) behavior cannot be studied with SAEs. Nonlinear activations are a major limitation because 1) they introduce complicated interactions between input features and 2) the neurons act as a preferred basis, so we cannot transform to the feature basis and cannot easily work with linear combinations of neurons. Ideally, we'd be able to derive features from weights themselves.
% Need to bridge somehow
%Another approach is to use a more interpretable architecture. \cite{bilinear_note} suggests that transformers featuring bilinear layers \cite{minh} have advantages for interpretability. A comparison of activations found that bilinear activations outperformed ReLU and GELU in transformer models \cite{shazeer2020glu}, and have similar performance to SwiGLU, which is used in LLaMA and PaLM models \cite{llama, palm}. Additionally, computations can be expressed in terms of linear operations with a third order tensor. This means we can leverage tensor or matrix decompositions to understand the weights. For other activation functions, 



%Our contributions are as follows:

%\begin{enumerate}
    %\item We describe a theoretic framework to interpret bilinear layers and discuss their properties. % good
%    \item We introduce the symmetric B tensor.
    % Separately, Lee Sharkey also introduces the B tensor. Does this mean we should include math in the introduction? Nah.
    %1. Introduction
    %2. Bilinear layers (refactoring Lee's note & introduce central object: the symmetric B tensor)
    %3. 
%    \item We use spectral analysis and sparse sensing to reveal the most important components of multi-layer models.
%    \item We open source our code (currently in supplementary material).
%\end{enumerate}

==> files/intro_michael.tex <==
%Although sparse auto-encoders (SAE) have had success, they depend on an additional training run (costly) and their features might depend on the dataset used. It is possible that out-of-distribution (OOD) behavior cannot be studied with SAEs. 
%Multi-Layer Perceptron
Nonlinear activations are a major limitation because 1) they introduce complicated interactions between input features and 2) the neurons act as a preferred basis, so we cannot transform to the feature basis and cannot easily work with linear combinations of neurons. Although sparse auto-encoders (SAE) have had success, they depend on an additional training run (costly) and their features might depend on the dataset used. It is possible that out-of-distribution (OOD) behavior cannot be studied with SAEs. Ideally, we'd be able to derive features from weights themselves.

Another approach is to use a more interpretable architecture. \cite{bilinear_note} suggests that transformers featuring bilinear layers \cite{minh} have advantages for interpretability. A comparison of activations found that bilinear activations outperformed ReLU and GELU in transformer models \cite{shazeer2020glu}, and have similar performance to SwiGLU, which is prevalent in competitive open source transformers today. Additionally, computations in bilinear layers can be expressed in terms of linear operations with a third order tensor. This means we can leverage tensor or matrix decompositions to understand the weights. For other activation functions, 

This paper aims to provide a detailed demonstration of extracting functionally relevant and interpretable features from model parameters alone, enabling static decompilation of deep neural networks. Concretely, we take one-layer and two-layer bilinear MLPs trained to classify MNIST digits, and decompose their weights into a set of eigenvectors that comprehensively explain model prediction.

Our contributions are as follows:

\begin{enumerate}
    \item We introduce a method to decompile bilinear MLPs and demonstrate it for shallow MNIST models and a small language model.
    \item We find that small models are \emph{not pathological} and learn crisp abstractions, contrary to some hypotheses.
    \item We show that existing foundation models can be finetuned into bilinear models using negligible data compared to pretraining.
\end{enumerate}
We open source our code and provide notebooks to replicate all experiments (currently in supplementary material).

==> files/intro_thomas.tex <==
% This is a quick outline of how I would write the introduction

Despite their necessity, non-linear activation functions have posed a major limitation to interpretability research. This stems from their imposition of a privileged basis in which input features interact deterministically, but not predictably. The activation of an output feature depends on both the weights and input. Consequently, the vast majority of interpretability techniques are input-dependent \citep{bau2020units, karpathy2015visualizing, Selvaraju_2019}. While these techniques have revealed considerable insight into the inner workings of models, they have no guarantees on out-of-distribution (OOD) data. Sparse Auto-Encoders (SAEs) have emerged as a promising direction to solve this issue through dictionary learning. However, recent work indicates that this approach also exhibits signs of input dependence [ref] and may not reveal grounded features in a model [ref]. Consequently, detecting harmful behaviors is unattainable without directly considering them in the input data. This poses a major safety issue that is becoming increasingly important to solve.

Recently, \citet{bilinear_note} suggested that bilinear layers \citep{shazeer2020glu} have desirable properties for weight-based interpretability. A direct accuracy comparison found that bilinear layers outperformed GELU-based units in transformer models \citep{shazeer2020glu}, and have similar performance to SwiGLU, which is used in contemporary frontier models (\citet{llama2, palm2}, inter alia). Importantly, computations in bilinear layers can be expressed in terms of linear operations with a third-order tensor. This opens the possibility to leverage tensor or matrix decompositions to understand the weights. 

This paper aims to demonstrate the viability of this approach by extracting functionally relevant and interpretable features from model parameters alone, enabling static decompilation of deep neural networks. Concretely, we study small image classification models up to two bilinear layers, trained on MNIST and Fashion-MNIST. We decompose their weights into a set of eigenvectors that comprehensively explain model prediction. Furthermore, we apply this approach to single-layer, transformer-based language models by replacing the MLPs with their bilinear counterparts. We study the inner workings of these MLPs and their impact on the final predictions through bigram analysis and eigendecompositions. Finally, we describe an efficient fine-tuning technique to convert existing models into bilinear versions.

Our contributions are as follows:
\begin{itemize}
    % \item We present bilinear layers and outline how they can serve as an interpretable replacement for ordinary activation functions.
    \item We introduce a method to decompose bilinear networks and show that it yields interpretable features for shallow MNIST models and a small language model.
    \item We show it is possible to fine-tune foundation models into a bilinear version using very little data without loss of accuracy.
    % \item We uncover several novel insights into the inner workings of small language models.
    % \item We open source our code (currently in supplementary material).
\end{itemize}



==> files/related_work.tex <==
\section{Related Work} \label{sec:related}

% Alice scratch pad

This work comes out of an emerging field of mechanistic interpretability. % cite transformer circuits

% TOPICS


Fully explaining the output of the model for a specific sample has been a deeply studied topic in interpretability research. Despite this, doing so remains exceedingly difficult. A recent study has shown that the underlying reason may be due to feature superposition. Concretely, they argue that a model represents more features than it has neurons and that there is therefore interference. Furthermore, (detrimentally) they show that these features may not even be basis-aligned, meaning that this information may be stored across a wide range of neurons that all interact in complex ways.

Using sparse autoencoders (SAEs) has proven to be the most promising avenue to disentangle these features. Unlike ordinary autoencoders, which typically aim to compress certain information into a more narrow space, SAEs project into a higher dimensional space. However, a strong sparsity penalty (typically L1) is applied such that learned representations are as sparse as possible. Intuitively, SAEs aim to extract the true features from entangled/superposed representations. Within LMs, this technique has been shown to produce more interpretable features. Unfortunately, it's still unclear if the features SAEs discover, correspond to those used for computation in the models. For example, SAEs may capture additional features based on the statistics of their training data. 

One further challenge to this technique is that there is no mapping between these features across layers. For instance, given two trained SAEs on representations from two adjacent layers, there is no way to directly trace the correspondence of features. To this end, recent work has focused on the training of "transcoders", which operate similarly to SAEs but instead aim to reveal interactions. Recently this process of extracting these features and their interactions has been referred to as "decompiling" the model. Currently, the non-linearities in models (and SAEs) make this complicated and noisy because many features interact in complicated ways. Despite these challenges, extracting true features from the model is an undeniably useful tool. 

The design choice to use bilinear layers obviates the need for transcoders. Essentially, the lack of non-linearity allows exact tracing of the SAE feature interactions onto the next layer. Furthermore [ref] suggests bilinear layers also possess desirable properties to understand single-layer transformers using the same principles.
